Combinatorial Approximations for Cluster Deletion: Simpler, Faster, and Better

Cluster deletion is an NP-hard graph clustering objective with applications in computational biology and social network analysis, where the goal is to delete a minimum number of edges to partition a graph into cliques. We first provide a tighter analysis of two previous approximation algorithms, improving their approximation guarantees from 4 to 3. Moreover, we show that both algorithms can be derandomized in a surprisingly simple way, by greedily taking a vertex of maximum degree in an auxiliary graph and forming a cluster around it. One of these algorithms relies on solving a linear program. Our final contribution is to design a new and purely combinatorial approach for doing so that is far more scalable in theory and practice.

==> content-arxiv/lp-solver-v0.tex <==
\section{Combinatorial Solver for the STC-LP}\label{sec:stc_lp_combinatorial}

In \autoref{sec:stc_lp_3_aprox} we have showed that the \cd problem can also be approximated by solving the LP relaxation for \minstc (\ref{eq:minstc_lp}) and running the deterministic \pivot procedure.
Moreover, \citeauthor{veldt2022correlationstc}~\cite{veldt2022correlationstc} showed that we can obtain a randomized, but faster, approximation by using a simpler rounding and clustering through a randomized \pivot procedure. % (\autoref{alg:minstc_lp}).
However, solving the LP relaxation is still a bottleneck (both speed and memory-wise). In this section we present a combinatorial algorithm for solving the \minstc relaxation that is faster, more scalable and requires less resources, while providing the same lower bound.
Moreover, the new bottleneck is solving a \minstcut, which is a well-studied problem with many efficient algorithms.

% \begin{algorithm}[!ht]
% 	% \setstretch{1.2}
% 	\caption{Rounding the \minstc LP relaxation~\cite{veldt2022correlationstc}}
% 	\label{alg:minstc_lp}

% 	{\bf Input.} Graph \(G = (V,E)\)

% 	{\bf Output.} Feasible \cd clustering of \(G\)

% 	\begin{algorithmic}[1]
% 		\STATE Solve LP relaxation (\ref{eq:minstc_lp}) of \minstc (\ref{eq:minstc_blp})
% 		\STATE Set \(\hat{E} \gets \{ (i,j) \in E \colon z_{ij} < 1/2 \}\)
% 		\STATE {\bf return} \pivot(\(\hat{G} = (V, \hat{E})\))
% 	\end{algorithmic}
% \end{algorithm}

% In our experiments, we find that these less expensive LP relaxations are faster, while typically performing just as well as algorithms based on canonical relaxations.

In this section we will go through the steps leading to this combinatorial algorithm.
The main idea of the algorithm is to reduce the \minstc LP relaxation to a \minstcut. This is done by converting the LP relaxation into a monotone IP2 problem and applying a simplification of \citeauthor{hochbaumApplications2021}'s reduction to the \closure problem~\cite{hochbaumApplications2021}.
The pseudocode for the combinatorial algorithm is presented in \autoref{alg:comb-stc-lp}. 
% todo this or the algorithm

\subsection{\minstc LP relaxation}

The LP relaxation of the \minstc binary LP (\ref{eq:minstc_blp}) is
\begin{equation}\label{eq:minstc_lp}
	\begin{array}{lll}
		\text{min}          & \displaystyle\sum\limits_{(i,j) \in E} x_{ij} \\
		\text{s.t.}   & x_{jk}  + x_{ik} \geq 1 & \text{if } (i,j,k) \in \wedges_k\\
		& 0 \leq x_{ij} \leq 1 & \forall (i,j) \in E \\
	\end{array}
\end{equation}

\begin{obser}\label{obs:half_integral}
	The LP relaxation (\ref{eq:minstc_lp}) is a half-integral LP, i.e., there exists an optimal solution that satisfies \(x_{ij} \in \{0, 1/2, 1\}\).
\end{obser}
This follows from the fact that the LP relaxation for vertex cover is half-integral~\cite{vazirani_rounding_2003}.

\subsection{Monotonization}

We first convert (\ref{eq:minstc_lp}) into a monotone IP2 problem.
For each \(x_{ij} \in [0,1]\), we create two variables \(x_{ij}^+ \in [0,1], x_{ij}^- \in [-1, 0]\) such that
\begin{equation}\label{x_plus_minus}
	x_{ij} = \frac{x_{ij}^+ - x_{ij}^-}{2}
\end{equation}

Then, the resulting LP is
\begin{equation}\label{minstc_lp_monotone}
	\begin{array}{lll}
		\text{min}          & \displaystyle\sum\limits_{(i,j) \in E} \frac{1}{2} x_{ij}^+ - \frac{1}{2} x_{ij}^- \\
		\text{s.t.}   & \left. \begin{aligned}
			x_{jk}^+  - x_{ik}^- \geq 1 \\
			x_{ik}^+  - x_{jk}^- \geq 1 \\
		\end{aligned} \right\} & \text{if } (i,j,k) \in \wedges_k\\
		& \left. \begin{aligned}
			0 \leq x_{ij}^+ \leq 1 \\
			-1 \leq x_{ij}^- \leq 0 \\
		\end{aligned} \right\} & \forall (i,j) \in E \\
	\end{array}
\end{equation}

\begin{obser}
	(\ref{minstc_lp_monotone}) is an integer LP, i.e., there is an optimal solution such that \(x_{ij}^+ \in \{0,1\}\) and \(x_{ij}^- \in \{-1,0\}\) for every \((i,j) \in E\).
\end{obser}

\begin{proof}
	Every row of the constraint matrix has exactly one 1 and one -1. Therefore, the constraint matrix is totally unimodular, so there is an integer optimal solution.
\end{proof}

We will show that solving the integer LP (\ref{minstc_lp_monotone}) is equivalent to solving (\ref{eq:minstc_lp}).

\begin{lemma}\label{th:opt_monotone_leq_lp}
	The optimal solution to LP (\ref{eq:minstc_lp}) is at most the optimal solution to LP (\ref{minstc_lp_monotone}), i.e., \(OPT_{\ref{eq:minstc_lp}} \leq OPT_{\ref{minstc_lp_monotone}}\).
\end{lemma}
\begin{proof}
	Observe that the objective function for both LPs is the same. Therefore, we just have to prove that, given a feasible solution \(\{x_{ij}^+, x_{ij}^-\}_{(i,j) \in E}\) to (\ref{minstc_lp_monotone}), we can construct a feasible solution \(\{x_{ij}\}_{(i,j) \in E}\) to (\ref{eq:minstc_lp}).
	For each \((i,j,k) \in \wedges\), let us refer to \(x_{jk}\) as \(x_1\) and \(x_{ik}\) as \(x_2\).
	Using \eqref{x_plus_minus} on LP (\ref{eq:minstc_lp}), we can rewrite its constraint for each wedge as 
	\begin{gather*}
		x_{1} + x_{2} \geq 1 \\
		\frac{x_{1}^+ - x_{1}^-}{2} + \frac{x_{2}^+ - x_{2}^-}{2} \geq 1 \\
		(x_{1}^+ - x_{2}^-) + (x_{2}^+ - x_{1}^-) \geq 2 \\
	\end{gather*}
	Observe that, if \(x_{ij}^+, x_{ij}^-\) satisfies the constraints of (\ref{minstc_lp_monotone}), then \(x_{ij}\) satisfies the constraints of (\ref{eq:minstc_lp}).
	
	We have proven that any feasible solution to (\ref{minstc_lp_monotone}) is also feasible for (\ref{eq:minstc_lp}), and the objective functions are equivalent, so \(OPT_{\ref{eq:minstc_lp}} \leq OPT_{\ref{minstc_lp_monotone}}\).
\end{proof}

\begin{lemma}\label{th:opt_monotone_geq_lp}
	If \(\{x_{ij}\}_{(i,j) \in E}\) is a half-integral feasible solution for LP (\ref{eq:minstc_lp}), then we can construct a binary feasible solution \(\{x_{ij}^+, x_{ij}^-\}_{(i,j) \in E}\) for LP (\ref{minstc_lp_monotone}) such that both LPs have the same objective function.
\end{lemma}
\begin{proof}
	First remember that (\ref{eq:minstc_lp}) is a half-integral LP and (\ref{minstc_lp_monotone}) is an integer LP.
	The variables \(\{x_{ij}^+, x_{ij}^-\}_{(i,j) \in E}\) will be constructed as follows:
	\begin{align*}
		x_{ij}=1 &\implies x_{ij}^+ = 1, x_{ij}^- = -1 \\
		x_{ij}=0 &\implies x_{ij}^+ = 0, x_{ij}^- = 0 \\
		x_{ij}=\frac{1}{2} &\implies x_{ij}^+ = 1, x_{ij}^- = 0 \\
	\end{align*}
	The fact that \(x_{ij} = (x_{ij}^+ - x_{ij}^-)/{2}\) is readily verified. We just need to prove that, if \(\{x_{ij}\}_{(i,j) \in E}\) is feasible for LP (\ref{eq:minstc_lp}), then \(\{x_{ij}^+, x_{ij}^-\}_{(i,j) \in E}\) is feasible for LP (\ref{minstc_lp_monotone}).
	To do so, take an arbitrary edge \((j,k) \in E\) and its half-integral LP variable \(x_{jk} \in \{0,1,1/2\}\).
	We will show that in all three cases, all constraints for LP (\ref{minstc_lp_monotone}) are satisfied.
	\begin{enumerate}[label=Case \arabic*:]
		\item \(x_{jk} = 1\).
		
		Then \(x_{jk}^+ = 1\) and \(x_{jk}^- = -1\), and each constraint pair for \((i,j,k) \in \wedges\) is satisfied, since \(x_{jk}^+ - x_{ik}^- = 1 - x_{ik}^- \geq 1\) and \(x_{ik}^+ - x_{jk}^- = x_{ik}^+ - (-1) \geq 1\).
		
		\item \(x_{jk} = 0\).
		
		Then \(x_{jk}^+ = 0\) and \(x_{jk}^- = 0\), and we know that, for each \((i,j,k) \in \wedges\), \(x_{ik}=1\). Thus, \(x_{ik}^+ = 1\) and \(x_{ik}^- = -1\), and the constraints for LP (\ref{minstc_lp_monotone}) are satisfied.
		
		\item \(x_{jk} = \frac{1}{2}\).
		
		Then \(x_{jk}^+ = 1\) and \(x_{jk}^- = 0\), and we know that, for each \((i,j,k) \in \wedges\), either \(x_{ik}=\frac{1}{2}\) or \(x_{ik}=1\). 
		(1) If \(x_{ik}=\frac{1}{2}\), then \(x_{ik}^+ = 1\) and \(x_{ik}^- = 0\), and the constraints for LP (\ref{minstc_lp_monotone}) are satisfied
		(2) If \(x_{ik}=1\), then \(x_{ik}^+ = 1\) and \(x_{ik}^- = -1\), and the constraints are satisfied once again.
	\end{enumerate}
	% \textit{Case 1:} \(x_{jk} = 1\).
	%
	% Then \(x_{jk}^+ = 1\) and \(x_{jk}^- = -1\), and each constraint pair for \((i,j,k) \in \wedges\) is satisfied, since \(x_{jk}^+ - x_{ik}^- = 1 - x_{ik}^- \geq 1\) and \(x_{ik}^+ - x_{jk}^- = x_{ik}^+ - (-1) \geq 1\).
	%
	% \textit{Case 2:} \(x_{jk} = 0\).
	%
	% Then \(x_{jk}^+ = 0\) and \(x_{jk}^- = 0\), and we know that, for each \((i,j,k) \in \wedges\), \(x_{ik}=1\). Thus, \(x_{ik}^+ = 1\) and \(x_{ik}^- = -1\), and the constraints for LP (\ref{minstc_lp_monotone}) are satisfied.
	%
	% \textit{Case 3:} \(x_{jk} = \frac{1}{2}\).
	%
	% Then \(x_{jk}^+ = 1\) and \(x_{jk}^- = 0\), and we know that, for each \((i,j,k) \in \wedges\), \(x_{ik}=\frac{1}{2}\). Thus, \(x_{ik}^+ = 1\) and \(x_{ik}^- = 0\), and the constraints for LP (\ref{minstc_lp_monotone}) are satisfied once again.
\end{proof}

\begin{theorem}
	The optimal value for LP (\ref{eq:minstc_lp}) equals the optimal value for LP (\ref{minstc_lp_monotone}), i.e., \(OPT_{\ref{eq:minstc_lp}} = OPT_{\ref{minstc_lp_monotone}}\).
\end{theorem}
\begin{proof}
	Since every half-integral solution to LP (\ref{eq:minstc_lp}) gives a feasible solution to LP (\ref{minstc_lp_monotone}) (\autoref{th:opt_monotone_geq_lp}) and the objective functions are equivalent, we know that \(OPT_{\ref{minstc_lp_monotone}} \leq OPT_{\ref{eq:minstc_lp}}\).
	However, \autoref{th:opt_monotone_leq_lp} already showed that \(OPT_{\ref{eq:minstc_lp}} \leq OPT_{\ref{minstc_lp_monotone}}\), therefore \(OPT_{\ref{eq:minstc_lp}} = OPT_{\ref{minstc_lp_monotone}}\).
\end{proof}

\subsection{Reduction to Closure Problem}

Next, we will reduce LP (\ref{minstc_lp_monotone}) into a closure problem. Given a vertex-weighted directed graph \(G=(V,E)\) and vertex weights \(\{w_i\}_{i \in V}\), the \closure problem tries to find a closed set \(V' \subseteq V\) (i.e., subset of vertices \(V'\) such that no edges leave \(V'\)) with maximum total weight.
The \closure problem can be formulated as an integer problem as follows:
\begin{equation*}\label{eq:closure}
	\begin{array}{lll}
		\text{max}          & \displaystyle\sum\limits_{i \in V} w_i x_i \\
		\text{s.t.}   		&  x_i \leq x_j & \forall (i,j) \in E \\
		& x_i \in \{0,1\} & \forall i \in V \\
	\end{array}
\end{equation*}

To convert LP (\ref{minstc_lp_monotone}) into a closure problem, we will change the LP to maximize the objective and substitute the variables \(\{x_{ij}^+, x_{ij}^-\}_{(i,j) \in E}\) for 0--1 variables \(\{x_{ij}^{++}, x_{ij}^{--}\}_{(i,j) \in E} \in \{0,1\}\). This substitution can be achieved thanks to LP (\ref{minstc_lp_monotone}) being an integer LP.
\begin{gather*}
	x^+ = 0 + x^{++} \\
	x^- = -1 + x^{--}
\end{gather*}
% todo esto se puede hacer?

The resulting maximization problem is the following:
\begin{equation}\label{eq:minstc_lp_closure}
	\begin{array}{lll}
		\text{max}          & \displaystyle\sum\limits_{(i,j) \in E} \frac{-1}{2} x_{ij}^{++} + \frac{1}{2} x_{ij}^{--} - \frac{1}{2} & \\
		\text{s.t.}   & \left. \begin{aligned}
			x_{ik}^{--} \leq x_{jk}^{++} \\
			x_{jk}^{--} \leq x_{ik}^{++} \\
		\end{aligned} \right\} \qquad \text{if } (i,j,k) \in \wedges_k &\\
		& x_{ij}^{++}, x_{ij}^{--} \in \{0,1\} \quad \forall (i,j) \in E &\\
		% & \left. \begin{aligned}
		% 	x_{ij}^{++} \in \{0,1\} \\
		% 	x_{ij}^{--} \in \{0,1\} \\
		% \end{aligned} \right\} \forall (i,j) \in E &\\
	\end{array}
\end{equation}

\subsection{Closure Problem to Min s-t Cut}

The closure problem can be solved efficiently with a minimum s-t cut on a related graph \(G_{st}\) \cite{picard_maximal_1976}. A proof of this reduction can be found by \citeauthor{hochbaumApplications2021}~\cite{hochbaumApplications2021}. 

The graph \(G_{st}\) will be a flow graph with all finite capacity arcs adjacent only to either the source or the sink.
Before constructing \(G_{st}\), we can simplify the objective function of (\ref{eq:minstc_lp_closure}) which will allow us to simplify the graph \(G_{st}\) (the finite-weight edges will have weight 1):
\begin{align*}
	&\argmax \sum\limits_{(i,j) \in E} \frac{-1}{2} x_{ij}^{++} + \frac{1}{2} x_{ij}^{--} - \frac{1}{2} \\
	= &\argmax \sum\limits_{(i,j) \in E} -1 \cdot x_{ij}^{++} + 1 \cdot x_{ij}^{--}
\end{align*}

The graph $G_{st}$ is constructed by creating nodes $x_{ij}^{++}, x_{ij}^{--}$ for each $(i,j) \in E$ and adding source and sink nodes, denoted as $s$ and $t$, respectively. 
The edges of the graph are formed by creating an infinite weight edge from $x_{ik}^{--} \rightarrow x_{jk}^{++}$ and from $x_{jk}^{--} \rightarrow x_{ik}^{++}$ for each $(i,j,k) \in \wedges_k$, and creating an edge with weight 1 from $s \rightarrow x_{ij}^{--}$ and from $x_{ij}^{++} \rightarrow t$ for each $(i,j) \in E$. 

To understand how \(G_{st}\) relates to LP (\ref{eq:minstc_lp_closure}) consider the following. The infinite weight edges enforce the constraints (\(x^{--} \leq x^{++}\)) by ensuring that if \(x^{--}=1\) then \(x^{++}=1\), i.e., if \(S\) is the source set solution of the \minstcut and \(x^{--} \in S\) then \(x^{++} \in S\).
The edges to the source and sink account for the objective function being optimized.

Given a solution to the \minstcut on $G_{st}$\footnote{%
	Notice that the objective for the \minstcut and the original LP relaxation does not have the same value due to the simplifications made. We can compute it by referring back to the original objective function in (\ref{eq:minstc_lp}).
}, with \(S\) being the source set, we can get back a solution to the closure problem by setting the LP variable \(x_{\cdot \cdot}^{\cdot \cdot} = 1\) if the node \(x_{\cdot \cdot}^{\cdot \cdot} \in S\), and \(x_{\cdot \cdot}^{\cdot \cdot} = 0\) otherwise.
We can then get back a half-integral optimal solution \(\{x_{ij}\}_{(i,j) \in E}\) for the original LP relaxation (\ref{eq:minstc_lp}) by reversing the substitutions
\begin{equation*}
	x_{ij} = \frac{1}{2} + \frac{x^{++} - x^{--}}{2}.
\end{equation*}

% Observe that if we rewrite the objective function as
% \begin{align*}
% 	\argmax \sum\limits_{(i,j) \in E} -1 \cdot x_{ij}^{++} + 1 \cdot x_{ij}^{--}
% 	&= \argmax \sum\limits_{(i,j) \in E} x_{ij}^{--} + (1-x_{ij}^{--}) - (1-x_{ij}^{--})  - x_{ij}^{++} \\
% 	&= \argmax \sum\limits_{(i,j) \in E} 1 - \sum\limits_{(i,j) \in E} [(1-x_{ij}^{--}) + x_{ij}^{++}] \\
% 	&= \argmin \sum\limits_{(i,j) \in E} (1-x_{ij}^{--}) + x_{ij}^{++} \\
% \end{align*}
% we can observe that the s-t cut is maximizing the number of \(x^{--}\) and minimizing the \(x^{++}\).

% If we relate this back to our original problem, 
% \begin{equation*}
% 	x = \frac{x^+ - x^-}{2} = \frac{x^{++} - x^{--}+1}{2}
% 	= \frac{1}{2} + \frac{x^{++} - x^{--}}{2}
% \end{equation*}

To understand how the \minstcut relates back to the original problem, consider the following.
Observe that \(x^{++}\) pushes edge \((i,j)\) towards being labeled as weak while \(x^{--}\) pushes it towards being labeled as strong.
Observe also that the \minstcut in \(G_{st}\) tries to include as many \(x^{--}\) into the source set as possible while excluding the \(x^{++}\). However, for each edge of a wedge, making the corresponding variable \(x^{--}=1\) (i.e., making it a strong edge) results in \(x^{++}=1\) (i.e., its partner edge being weak) due to the infinite weight edge. This results in a cost of 1. However, if given a wedge, both edges or neither are selected as strong edges, both will receive a value of \(1/2\) which, after rounding (\autoref{alg:minstc_lp}) results in both edges being labeled as weak. This results in a cost of 2.

\subsection{Summary Algorithm}

\autoref{alg:comb-stc-lp} combines all the steps, summarizing the combinatorial algorithm to find the optimal solution to the LP relaxation of the \textsc{MinSTC} problem, i.e., LP (\ref{eq:minstc_lp}). This algorithm combined with the rounding procedure from \autoref{alg:minstc_lp} provides an approximation to the \cd problem.

\begin{algorithm}[!ht]
	\caption{Combinatorial solver for \textsc{MinSTCut}-STC}
	\label{alg:comb-stc-lp}
	
	{\bf Input.} Graph \(G = (V,E)\)
	
	{\bf Output.} Optimal solution to the LP relaxation (\ref{eq:minstc_lp})
	
	\begin{algorithmic}[1]
		\STATE Create empty s-t graph \(G_{st}\)
		\STATE For each \((i,j) \in E\), add to \(G_{st}\) nodes \(x_{ij}^{++}, x_{ij}^{--}\)
		\STATE Add to \(G_{st}\) nodes \(s,t\)
		\STATE For each \((i,j,k) \in \wedges_k\), add to \(G_{st}\) an edge with infinite weight from \(x_{ik}^{--} \rightarrow x_{jk}^{++}\) and from \(x_{jk}^{--} \rightarrow x_{ik}^{++}\)
		\STATE For each \((i,j) \in E\), add to G an edge with weight 1 from \(s \rightarrow x_{ij}^{--}\) and from \(x_{ij}^{++} \rightarrow t\)
		\STATE \(S \gets\) source set of min s-t cut on \(G_{st}\)
		\STATE For each node \(z \in G\) and its corresponding variable \(x_{\cdot \cdot}^{\cdot \cdot}\), \(x_{\cdot \cdot}^{\cdot \cdot} = 1\) if \(z \in S\), \(x_{\cdot \cdot}^{\cdot \cdot}=0\) otherwise
		\STATE For each \((i,j) \in E\), \(x_{ij} = \frac{1}{2} + \frac{x_{ij}^{++} - x_{ij}^{--}}{2}\)
		
		\STATE \textbf{Return} \(\{x_{ij}\}_{(i,j) \in E}\)
	\end{algorithmic}
\end{algorithm}

==> content-arxiv/lp-solver-v1.tex <==
\section{Combinatorial Solver for the STC LP}\label{sec:stc_lp_combinatorial}
Although the STC LP rounding algorithm produces the same 3-approximation guarantee as MFP, the LP relaxation produces a tighter lower bound for \cd and tends to produce better solutions in practice. However, previous implementations rely on simply applying black-box LP solvers, which become a bottleneck both in terms of runtime and memory requirements~\cite{veldt2022correlation}. In this section we leverage the fact that the STC LP corresponds to the LP relaxation for a special type of vertex cover problem, and show it is amenable to a purely combinatorial and more efficient solver. We provide complete details showing how it can be cast as a so-called monotone IP2 problem~\cite{hochbaumApplications2021} and solved via reduction to a minimum $s$-$t$ cut problem.
The pseudocode for the combinatorial algorithm is presented in Algorithm~\autoref{alg:comb-stc-lp}. 


\subsection{Converting to Monotone IP2}
The STC LP relaxation is
\begin{equation}\label{eq:minstc_lp}
	\begin{array}{lll}
		\text{min}          & \sum_{(i,j) \in E} x_{ij} \\
		\text{s.t.}   & x_{jk}  + x_{ik} \geq 1 & \text{if } (i,j,k) \in \wedges_k\\
		& 0 \leq x_{ij} \leq 1 & \forall (i,j) \in E \\
	\end{array}
\end{equation}
Recall that every basic feasible solution is half-integral, so we could equivalently optimize over variables $x_{ij} \in \{0,1/2, 1\}.$ We will show that this is equivalent to the following optimization problem:
\begin{equation}\label{minstc_lp_monotone}
	\begin{array}{lll}
		\text{min}          & \displaystyle\sum\limits_{(i,j) \in E} \frac{1}{2} x_{ij}^+ - \frac{1}{2} x_{ij}^- \\
		\text{s.t.}   & \left. \begin{aligned}
			x_{jk}^+  - x_{ik}^- \geq 1 \\
			x_{ik}^+  - x_{jk}^- \geq 1 \\
		\end{aligned} \right\} & \text{if } (i,j,k) \in \wedges_k\\
		& \left. \begin{aligned}
			x_{ij}^+ \in \{0,1\} \\
			x_{ij}^- \in \{-1, 0\} \\
		\end{aligned} \right\} & \forall (i,j) \in E. \\
	\end{array}
\end{equation}
This latter problem is known as a monotone IP2 problem: an integer program in which every constraint involves two variables, which have coefficients with opposite signs~\cite{hochbaumApplications2021}. Although integer programming is NP-hard in general, monotone IP2 problems can be solved in polynomial time given their special structure.
% The constraint set in this latter problem is totally unimodular, meaning that every basic feasible solution is integral. This means we can restrict out attention to variables satisfying $x_{ij}^+ \{0,1\}$ and $x_{ij}^- \in \{-1, 0\}$ for every $(i,j) \in E$.

{\color{blue} I'll probably come back and actually replace this theorem with a proof that directly shows the STC LP is equivalent to~\eqref{eq:minstc_lp_closure}, which in turn is not hard to show is an s-t cut problem. -Nate}
\begin{theorem}
\label{thm:equiv}
    Let $\{x_{ij}^+, x_{ij}^-\}_{ij \in E}$ be an optimal solution for the problem in~\eqref{minstc_lp_monotone} and define 
    \begin{equation}\label{x_plus_minus}
	x_{ij} = \frac12x_{ij}^+ - \frac12x_{ij}^-.
\end{equation}
Then $\{x_{ij}\}_{ij \in E}$ is an optimal solution for the STC LP.
\end{theorem}
\begin{proof}
Let $\text{OPT}_\mathit{LP}$ denote the optimal solution to the STC LP relaxation and $\text{OPT}_\mathit{m}$ denote the optimal solution to the monotone IP2 problem in~\eqref{minstc_lp_monotone}. 

Let $\{x_{ij}^+, x_{ij}^-\}_{ij \in E}$ be feasible for the monotone IP2. The integer constraints on these variables and the definition of $x_{ij}$ in~\eqref{x_plus_minus} guarantee that $x_{ij} \in \{0,1/2, 1\}.$ The relationship between variables given in~\eqref{x_plus_minus} also shows that the objective functions for the two problems are equivalent. For a given $(i,j,k) \in \mathcal{W}_k$, adding the two constraints $x_{jk}^+  - x_{ik}^- \geq 1$ and $x_{ik}^+  - x_{jk}^- \geq 1$ produces the constraint $x_{jk} + x_{ik} \geq 1$. In other words, a feasible solution for the monotone IP2 problem leads to a feasible solution to the STC-LP with the same objective value, and hence $\text{OPT}_\mathit{LP} \leq \text{OPT}_\mathit{m}$.

Next, consider a half-integral feasible solution $\{x_{ij}\}_{ij \in E}$ for the STC LP and define
\begin{equation*}
(x_{ij}^+, x_{ij}^-) = 
\begin{cases}
        (1,-1) & \text{ if $x_{ij} = 1$} \\
        (0,0) & \text{ if $x_{ij} = 0$} \\   
        (1,0) & \text{ if $x_{ij} = 1/2$}. 
\end{cases}
\end{equation*}
One can check that this set of variables satisfies equation~\eqref{x_plus_minus} and will be feasible for the monotone IP2 problem, hence $\text{OPT}_\mathit{LP} \geq \text{OPT}_\mathit{m}$.
Combining both sides we have $\text{OPT}_\mathit{LP} = \text{OPT}_\mathit{m}$.
\end{proof}

\subsection{Reduction to Closure Problem}

Next, we will reduce LP (\ref{minstc_lp_monotone}) into a closure problem. Given a vertex-weighted directed graph \(G=(V,E)\) and vertex weights \(\{w_i\}_{i \in V}\), the \closure problem tries to find a closed set \(V' \subseteq V\) (i.e., subset of vertices \(V'\) such that no edges leave \(V'\)) with maximum total weight.
The \closure problem can be formulated as an integer problem as follows:
\begin{equation*}\label{eq:closure}
	\begin{array}{lll}
		\text{max}          & \displaystyle\sum\limits_{i \in V} w_i x_i \\
		\text{s.t.}   		&  x_i \leq x_j & \forall (i,j) \in E \\
		& x_i \in \{0,1\} & \forall i \in V \\
	\end{array}
\end{equation*}

To convert LP (\ref{minstc_lp_monotone}) into a closure problem, we will change the LP to maximize the objective and substitute the variables \(\{x_{ij}^+, x_{ij}^-\}_{(ij \in E}\) for 0--1 variables \(\{y_{ij}, z_{ij}\}_{ij\in E} \in \{0,1\}\) via the following substitution for each $(i,j) \in E$:
\begin{gather*}
	y_{ij} = x^+_{ij}  \text{ and } z_{ij} = x_{ij}^- + 1.
\end{gather*}
The objective function can then be written as 
\begin{align*}
    \min \sum_{(i,j) \in E} \frac{1}{2}y_{ij} - \frac12 z_{ij} + \frac12.
\end{align*}
Multiplying the objective by two we obtain the following equivalent problem
\begin{equation}\label{eq:minstc_lp_closure}
	\begin{array}{lll}
		\min        & \displaystyle\sum\limits_{(i,j) \in E} y_{ij} + (1- z_{ij}) & \\
		\text{s.t.}   & \left. \begin{aligned}
			z_{ik} \leq y_{jk} \\
			z_{jk} \leq y_{ik} \\
		\end{aligned} \right\} \qquad \text{if } (i,j,k) \in \wedges_k &\\
		& z_{ij}, y_{ij} \in \{0,1\} \quad \forall (i,j) \in E &
	\end{array}
\end{equation}

{\color{blue} Note that to simplify notation I have started to change $x_{ij}^{++} \rightarrow y_{ij}$ and $x_{ij}^{--} \rightarrow z_{ij}$, but haven't changed it everywhere yet. Actually though as noted before Theorem~\ref{thm:equiv}---while everything we have here going from the STC LP to a min-st-cut problem is correct, I believe we can also save space and make this simpler conceptually by drawing a more direct path from the STC LP to the resulting min-st-cut without going through all the intermediate steps. E.g., go from LP~\eqref{eq:minstc_lp} to~\eqref{eq:minstc_lp_closure} without explicitly talking about monotone IP2 problems and closure problems. I can work on streamlining this. We should also eventually nail down what the best runtime is for the resulting flow problem. It's a very special type of min-st-cut problem so I wonder if we can get a specialized runtime, but offhand I don't know what the best runtime will end up being. -Nate}
\begin{theorem}
\label{thm:equiv}
    Let $\{y_{ij}, z_{ij}\}_{ij \in E}$ be an optimal solution for the problem in~\eqref{eq:minstc_lp_closure} and define 
    \begin{equation}\label{x_plus_minus}
	x_{ij} = \frac12(y_{ij} - z_{ij} + 1).
\end{equation}
Then $\{x_{ij}\}_{ij \in E}$ is an optimal solution for the STC LP.
\end{theorem}
\begin{proof}
    To do. Follow the outline of the current proof for Theorem~\ref{thm:equiv}. 
\end{proof}
\subsection{Closure Problem to Min s-t Cut}
The closure problem can be reduced to a minimum $s$-$t$ cut on a related graph \(G_{st}\) \cite{picard_maximal_1976}. We follow the presentation given by~\citet{hochbaumApplications2021}. The graph \(G_{st}\) will be a flow graph with all finite capacity arcs adjacent only to either the source or the sink. It is constructed by creating one node for each variable $y_{ij}$ and each variable $z_{ij}$ for each $(i,j) \in E$ and adding source and sink nodes, denoted as $s$ and $t$, respectively. We abuse notation and let $z_{ij}$ and $y_{ij}$ represent nodes in the graph $G_{st}$ in addition to representing variables in LP~\eqref{eq:minstc_lp_closure}.
We introduce directed infinite weight edges from $z_{ik}$ to $y_{jk}$ and from $z_{jk}$ to $y_{ik}$ for each $(i,j,k) \in \wedges_k$. We then create an edge with weight 1 from $s$ to $z_{ij}$ and from $y_{ij}$ to $t$ for each $(i,j) \in E$. 

To understand how \(G_{st}\) relates to LP (\ref{eq:minstc_lp_closure}) consider the following. The infinite weight edges enforce the constraints (\(x^{--} \leq x^{++}\)) by ensuring that if \(x^{--}=1\) then \(x^{++}=1\), i.e., if \(S\) is the source set solution of the \minstcut and \(x^{--} \in S\) then \(x^{++} \in S\).
The edges to the source and sink account for the objective function being optimized.

Given a solution to the \minstcut on $G_{st}$\footnote{%
	Notice that the objective for the \minstcut and the original LP relaxation does not have the same value due to the simplifications made. We can compute it by referring back to the original objective function in (\ref{eq:minstc_lp}).
}, with \(S\) being the source set, we can get back a solution to the closure problem by setting the LP variable \(x_{\cdot \cdot}^{\cdot \cdot} = 1\) if the node \(x_{\cdot \cdot}^{\cdot \cdot} \in S\), and \(x_{\cdot \cdot}^{\cdot \cdot} = 0\) otherwise.
We can then get back a half-integral optimal solution \(\{x_{ij}\}_{(i,j) \in E}\) for the original LP relaxation (\ref{eq:minstc_lp}) by reversing the substitutions
\begin{equation*}
	x_{ij} = \frac{1}{2} + \frac{x^{++} - x^{--}}{2}.
\end{equation*}

% Observe that if we rewrite the objective function as
% \begin{align*}
% 	\argmax \sum\limits_{(i,j) \in E} -1 \cdot x_{ij}^{++} + 1 \cdot x_{ij}^{--}
% 	&= \argmax \sum\limits_{(i,j) \in E} x_{ij}^{--} + (1-x_{ij}^{--}) - (1-x_{ij}^{--})  - x_{ij}^{++} \\
% 	&= \argmax \sum\limits_{(i,j) \in E} 1 - \sum\limits_{(i,j) \in E} [(1-x_{ij}^{--}) + x_{ij}^{++}] \\
% 	&= \argmin \sum\limits_{(i,j) \in E} (1-x_{ij}^{--}) + x_{ij}^{++} \\
% \end{align*}
% we can observe that the s-t cut is maximizing the number of \(x^{--}\) and minimizing the \(x^{++}\).

% If we relate this back to our original problem, 
% \begin{equation*}
% 	x = \frac{x^+ - x^-}{2} = \frac{x^{++} - x^{--}+1}{2}
% 	= \frac{1}{2} + \frac{x^{++} - x^{--}}{2}
% \end{equation*}

To understand how the \minstcut relates back to the original problem, consider the following.
Observe that \(x^{++}\) pushes edge \((i,j)\) towards being labeled as weak while \(x^{--}\) pushes it towards being labeled as strong.
Observe also that the \minstcut in \(G_{st}\) tries to include as many \(x^{--}\) into the source set as possible while excluding the \(x^{++}\). However, for each edge of a wedge, making the corresponding variable \(x^{--}=1\) (i.e., making it a strong edge) results in \(x^{++}=1\) (i.e., its partner edge being weak) due to the infinite weight edge. This results in a cost of 1. However, if given a wedge, both edges or neither are selected as strong edges, both will receive a value of \(1/2\) which, after rounding (\autoref{alg:minstc_lp}) results in both edges being labeled as weak. This results in a cost of 2.

\subsection{Summary Algorithm}

\autoref{alg:comb-stc-lp} combines all the steps, summarizing the combinatorial algorithm to find the optimal solution to the LP relaxation of the \textsc{MinSTC} problem, i.e., LP (\ref{eq:minstc_lp}). This algorithm combined with the rounding procedure from \autoref{alg:minstc_lp} provides an approximation to the \cd problem.

\begin{algorithm}[!ht]
	\caption{Combinatorial solver for \textsc{MinSTCut}-STC}
	\label{alg:comb-stc-lp}
	
	{\bf Input.} Graph \(G = (V,E)\)
	
	{\bf Output.} Optimal solution to the LP relaxation (\ref{eq:minstc_lp})
	
	\begin{algorithmic}[1]
		\STATE Create empty s-t graph \(G_{st}\)
		\STATE For each \((i,j) \in E\), add to \(G_{st}\) nodes \(x_{ij}^{++}, x_{ij}^{--}\)
		\STATE Add to \(G_{st}\) nodes \(s,t\)
		\STATE For each \((i,j,k) \in \wedges_k\), add to \(G_{st}\) an edge with infinite weight from \(x_{ik}^{--} \rightarrow x_{jk}^{++}\) and from \(x_{jk}^{--} \rightarrow x_{ik}^{++}\)
		\STATE For each \((i,j) \in E\), add to G an edge with weight 1 from \(s \rightarrow x_{ij}^{--}\) and from \(x_{ij}^{++} \rightarrow t\)
		\STATE \(S \gets\) source set of min s-t cut on \(G_{st}\)
		\STATE For each node \(z \in G\) and its corresponding variable \(x_{\cdot \cdot}^{\cdot \cdot}\), \(x_{\cdot \cdot}^{\cdot \cdot} = 1\) if \(z \in S\), \(x_{\cdot \cdot}^{\cdot \cdot}=0\) otherwise
		\STATE For each \((i,j) \in E\), \(x_{ij} = \frac{1}{2} + \frac{x_{ij}^{++} - x_{ij}^{--}}{2}\)
		
		\STATE \textbf{Return} \(\{x_{ij}\}_{(i,j) \in E}\)
	\end{algorithmic}
\end{algorithm}

==> content-arxiv/scratch.tex <==
% Proof for Lemma 4.1 that's too long

We provide full details for proving Lemma~\ref{lem:equiv}, which rerestate here for convenience.
\nate{I wrote this out quickly--details should be double checked.}
\begin{lemma}
    % \label{lem:equiv}
If $\{y_{ij}, z_{ij} \}_{ij \in E}$ is feasible for the monotone IP2 problem in~\eqref{eq:ip}, then 
\begin{equation}\label{ip2lp}
	x_{ij} = \frac12(y_{ij} - z_{ij} + 1) \quad \forall(i,j) \in E
\end{equation}
defines a feasible half-integral solution for the STC LP with the same objective value. Conversely, if $\{x_{ij}\}_{ij \in E}$ is a feasible half-integral solution to the STC LP, the variables
\begin{equation}
    \label{LP2IP}
    (y_{ij}, z_{ij}) = 
    \begin{cases}
            (0,1) & \text{ if $x_{ij} = 0$} \\
            (1,1) & \text{ if $x_{ij} = 1/2$} \\   
            (1,0) & \text{ if $x_{ij} = 1$}. 
    \end{cases}
    \quad \forall(i,j) \in E
    \end{equation} 
    are feasible for the IP and have the same objective value.
\end{lemma}
\begin{proof}
Let $\text{OPT}_\mathit{LP}$ denote the optimal solution to the STC LP relaxation and $\text{OPT}_\mathit{IP}$ denote the optimal solution to the IP in~\eqref{eq:ip}. The integer constraints on variables $\{y_{ij}, z_{ij}\}_{ij \in E}$ and the definition of $x_{ij}$ 
in~\eqref{ip2lp} guarantee that $x_{ij} \in \{0,1/2, 1\}.$ The relationship between variables given in~\eqref{ip2lp} also shows that the objective functions for the two problems are equivalent. For a given $(i,j,k) \in \mathcal{W}_k$, the two constraints $y_{jk}  - z_{ik} \geq 0$ and $y_{ik}  - z_{jk} \geq 0$ and Eq.~\eqref{ip2lp} together imply
\begin{align*}
    & y_{jk} - z_{jk} + y_{ik} - z_{ik} \geq 0 \implies 2x_{jk} - 1 + 2x_{ik} -1 \geq 0 \implies x_{jk} + x_{ik} \geq 1.
\end{align*}
In other words, a feasible solution the IP leads to a feasible solution to the STC LP with the same objective value, and hence $\text{OPT}_\mathit{LP} \leq \text{OPT}_\mathit{IP}$. 

To show that this actually gives the optimal solution to the STC LP, we can use Eq.~\eqref{LP2IP} to show how to map from an arbitrary feasible solution to the STC LP to a feasible solution to the IP with the same objective value. To prove feasibility 
we consider an arbitrary 
% variable $x_{jk} \in \{0,1/2,1\}$ and show that all constraints involving this variable will be satisfied. In particular, we must show that for every $i$ such that 
open wedge $(i,j,k) \in \mathcal{W}_k$ and the two corresponding constraints.
\begin{align*}
    z_{ik} \leq y_{jk} \\
    z_{jk} \leq y_{ik}.
\end{align*}
We prove that these constraints will be satisfied via a case analysis on variable $x_{jk} \in \{0, 1/2, 1\}$.

\textbf{Case 1:} \(x_{jk} = 1\).
Then $y_{jk} = 1 \geq z_{ik}$ and $z_{jk} = 0 \leq y_{ik}$, so the constraints are satisfied.

\textbf{Case 2:} \(x_{jk} = 0\).
Then we know that \(x_{ik}=1\) for each \((i,j,k) \in \wedges\), so \(y_{ik} = 1 \geq z_{jk}\) and \(z_{ik} = 0 \leq y_{jk}\).
		
\textbf{Case 3:} \(x_{jk} = \frac{1}{2}\).
Then \(y_{jk} = 1\) and \(z_{jk} = 1\), and we know that, for each \((i,j,k) \in \wedges\), either \(x_{ik}=\frac{1}{2}\) or \(x_{ik}=1\). (1) If \(x_{ik}=\frac{1}{2}\), then \(y_{ik} = 1\) and \(z_{ik} = 1\), and the constraints are satisfied. (2) If \(x_{ik}=1\), then \(y_{ik} = 1\) and \(z_{ik} = 0\), and the constraints are satisfied once again.

This shows that $\text{OPT}_\mathit{LP} \geq \text{OPT}_\mathit{IP}$, and hence the optimal solutions coincide. 
\end{proof}


%% Saved pseudocode

\begin{algorithm}[t]
	\caption{Faster maximal edge-disjoint open wedge set}
	\label{alg:fow}
	\begin{algorithmic}[1]
 \STATE 	{\bf Input.} Graph $G = (V,E)$
\STATE {\bf Output.} Maximal edge-disjoint set of open wedges $W \subseteq \mathcal{W}(G)$
\STATE $W$ = \emptyset$   \quad \texttt{// edge-disjoint open wedge set}
\STATE $E_W = \emptyset$  \texttt{ //edges within W, will be labeled "weak"}
\FOR{$v \in V$} 
\STATE $N_v \leftarrow$ array of neighbors $u$ of $v$ such that $(u,v) \notin E_W$
\IF{$|N_v| < 2$}
\STATE continue \texttt{ // no open wedges centered at $v$}
\ENDIF
\STATE $U = [2, 3, \cdots , |N_v|, \mathit{END}]$  \hfill \texttt{ // $U[t] = $ neighbor of $v$ to visit after the $t$-th neighbor}
\STATE $i = 1$; $j = 2$
\STATE $\text{stillprocessing} = \text{TRUE}$
\WHILE{$\text{stillprocessing} = \text{TRUE}$}
\STATE $v_i = N_v[i]$; $v_j = N_v[j]$ \hfill \texttt{// $(v_i, v_j, v)$ is current wedge under consideration}
\IF{$(v_i, v_j) \in E$}
\STATE $T = T + 1$ \hfill \texttt{// triangle found; do normal increment}
\IF{$U[j] \neq \text{END}$}
\STATE $j_\mathit{old} = j$ \hfill \texttt{// record $j_\mathit{old}$ such that $U[j_\mathit{old}] == j$}
\STATE  $j = U[j]$ \hfill \texttt{ // increment $j$}
\ELSIF{$U[j] == \text{END}$ and $U[i] \neq j$}
\STATE $i = U[i]$\hfill \texttt{// increment $i$}
\STATE $j = U[i]$ 
\ELSE
$\text{stillprocessing} = \text{FALSE}$ \hfill \texttt{// done exploring neighbors since  $j = U[i]$ and $U[j] == \text{END}$}
\ENDIF
\ELSE
% \STATE $i = U[i]$ \hfill \texttt{// increment $i$}
\STATE $O = O + 1$ \hfill \texttt{// open wedge found; do special increment}
\STATE $E_W \leftarrow E_W \cup \{(v,v_j), (v,v_i) \}$
\STATE $W \leftarrow W \cup \{(v_i, v_j, v) \}$
\IF{$j == U[i]$}
\STATE $i = U[j]$ \hfill \texttt{$i$ and $j$ were consecutive, increment $i$ past both}
\ELSE
\STATE $U[j_\mathit{old}] = U[j]$ \hfill \texttt{ // skip past $(v,v_j)$ in the future}
\STATE $i = U[i]$ \hfill \texttt{// increment $i$}
\ENDIF
\IF{$i == \text{END}$ or $U[i] == \text{END}$}
\STATE $\text{stillprocessing} = \text{FALSE}$
\ELSE $j = U[i]$
\ENDIF
\ENDIF
\ENDWHILE
\ENDFOR
\STATE \textbf{Return} $W$
\end{algorithmic}
\end{algorithm}


%% Save old version:

Algorithm~\ref{alg:fow} provides pseudo-code for our $O(|E|^{1.5})$-time algorithm for finding a maximal edge-disjoint set of open wedges in a graph. 
\begin{algorithm}[t]
	\caption{Faster maximal edge-disjoint open wedge set}
	\label{alg:fow}
	\begin{algorithmic}[1]
 \STATE 	{\bf Input.} Graph $G = (V,E)$
\STATE {\bf Output.} Maximal edge-disjoint set of open wedges $W \subseteq \mathcal{W}(G)$
\STATE $E_W = \emptyset$  \texttt{ //edges within W, will be labeled "weak"}
\FOR{$v \in V$} 
\STATE $N_v \leftarrow$ array of neighbors $u$ of $v$ such that $(u,v) \notin E_W$
\IF{$|N_v| < 2$}
\STATE continue \texttt{ // no open wedges centered at $v$}
\ENDIF
\STATE $U = [2, 3, \cdots , |N_v|, \mathit{END}]$  \hfill \texttt{ // $U[t] = $ neighbor of $v$ to visit after the $t$-th neighbor}
\STATE $i = 1$; $j = 2$
\STATE $\text{stillprocessing} = \text{TRUE}$
\WHILE{$\text{stillprocessing} = \text{TRUE}$}
\STATE $v_i = N_v[i]$; $v_j = N_v[j]$ \hfill \texttt{// $(v_i, v_j, v)$ is current wedge under consideration}
\IF{$(v_i, v_j) \in E$}
\STATE $T = T + 1$ \hfill \texttt{// triangle found; do normal increment}
\IF{$U[j] \neq \text{END}$}
\STATE $j_\mathit{old} = j$ \hfill \texttt{// record $j_\mathit{old}$ such that $U[j_\mathit{old}] == j$}
\STATE  $j = U[j]$ \hfill \texttt{ // increment $j$}
\ELSIF{$U[j] == \text{END}$ and $U[i] \neq j$}
\STATE $i = U[i]$\hfill \texttt{// increment $i$}
\STATE $j = U[i]$ 
\STATE $j_\mathit{old} = i$
\ELSE
$\text{stillprocessing} = \text{FALSE}$ \hfill \texttt{// done exploring neighbors since  $j = U[i]$ and $U[j] == \text{END}$}
\ENDIF
\ELSE
\STATE $O = O + 1$ \hfill \texttt{// open wedge found; do special increment}
\STATE $E_W \leftarrow E_W \cup \{(v,v_j), (v,v_i) \}$
\STATE $W \leftarrow W \cup \{(v_i, v_j, v) \}$
\STATE $U[j_\mathit{old}] = U[j]$ \hfill \texttt{ // skip past $(v,v_j)$ in the future}
\STATE $i = U[i]$ \hfill \texttt{// increment $i$}
\IF{$i == \text{END}$ or $U[i] == \text{END}$}
\STATE $\text{stillprocessing} = \text{FALSE}$
\ELSE $j = U[i]$
\ENDIF
\ENDIF
\ENDWHILE
\ENDFOR
\STATE \textbf{Return} $W$
\end{algorithmic}
\end{algorithm}

%% Old text from abstract

	% Cluster deletion is an NP-hard graph modification problem where the goal is to delete as few edges as possible such that every connected component of the resulting graph is a clique. The problem was first motivated by applications in computational biology, and has since been studied extensively from the perspective of approximation algorithms and fixed-parameter tractability results. Existing approximation algorithms for this problem rely either on expensive linear programming relaxations or faster combinatorial algorithms with weaker lower bounds. We provide contributions on both fronts. First, we improve the best approximation factor for a \emph{purely combinatorial} algorithm from 4 to 3, by significantly simplifying the presentation of an existing method and using a more careful proof technique. We also provide a purely combinatorial approach for solving a linear programming relaxation (LP) of the problem---which comes with a tighter lower bound---by showing how to reduce it to a minimum $s$-$t$ cut problem. We additionally improve the approximation factor for rounding this LP. These results provide a much deeper understanding of combinatorial techniques for cluster deletion and enable us in practice to solve the LP relaxation on a far larger scale than was previously possible.
 Cluster deletion is an NP-hard graph clustering objective with applications in computational biology and social network analysis, where the goal is to delete a minimum number of edges to partition a graph into cliques. 
 % Several approximation algorithms for the problem have been designed previously, but many of these rely on expensive linear programming relaxations and are not combinatorial.
 % Furthermore, the best deterministic approximation algorithms rely on complicated and expensive techniques for derandomizing simpler randomized algorithms.
 We present several contributions in terms of simple and fast combinatorial approximation algorithms.
 We first provide a tighter analysis of two previous algorithms, improving their approximation guarantees from 4 to 3.
 One of these algorithms relies on solving a linear programming relaxation; another of our contributions is to design a new and purely combinatorial approach for doing so that is far more scalable both in theory and practice. 
 Finally, we provide a simple new technique for derandomizing randomized algorithms for the problem, that is far simpler and faster than previous deterministic algorithms for cluster deletion.

 Moreover, we show that both algorithms can be derandomized in a surprisingly simple way, greedily taking a vertex of the maximum degree in an auxiliary graph as the pivot.

 {\color{violet}
  The original proof.
\begin{proof}
  We begin by proving that for every choice of pivot nodes in $\hat{G}$, at most half of the edges in $E_h$ will end up inside the clusters formed by Algorithm~\ref{alg:stclp_rounding}. To prove this, let ${\mathcal{B}}_h$ be the set of half-edges between clusters and ${\mathcal{N}}_h$ the set of half-edges inside clusters resulting from an arbitrary choice of pivots. Define a new set of binary variables $\{\hat{x}_{ij}\}_{ij \in E}$, which we will prove is still feasible for the LP, by
  \begin{align*}
    \hat{x}_{ij} = \begin{cases}
      x_{ij} & \text{ if $x_{ij} \in \{0,1\}$} \\
      1 & \text{ if $x_{ij} \in {\mathcal{B}}$}_h \\
      0  & \text{ if $x_{ij} \in {\mathcal{N}}$}_h.
    \end{cases}
  \end{align*}
  % We prove this set of variables is still feasible for the LP. 
 Consider an arbitrary open wedge $(i,j,k) \in \wedges(G)$. If either one of the variables $x_{ik}$ and $x_{jk}$ is in $\{0,1\}$, then at least one of them equals 1 and so $\hat{x}_{ik} + \hat{x}_{jk} \geq 1$. Assume then that both $(i,k)$ and $(j,k)$ are half-edges. It is impossible for both of them to be in ${\mathcal{N}}_h$ since that would imply $i$ and $j$ are both clustered with $k$ and hence clustered with each other, contradicting Observation~\ref{lem:cliques}. If on the other hand at least one of them is in ${\mathcal{B}}_h$, then $\hat{x}_{ik} + \hat{x}_{jk} \geq 1$. 
 We claim now that $|{\mathcal{B}}_h| \geq |{\mathcal{N}}_h|$. If this were not the case, then the feasible variables $\{\hat{x}_{ij}\}$ would have a strictly smaller LP objective value, contradicting the optimality of $\{x_{ij}\}$.
	
	Let $M_1$ be the number of mistakes at $E_1$ edges, $M_h$ be the number of mistakes at half-edges $E_h$, and $M_S$ be the number of strong edge mistakes. Using Pivot Strategy 1 or 2, Lemma~\ref{lem:piv} implies that $M_S \leq 2( |E_1| - M_1 + |E_h| - M_h)$. We can then bound the total number of mistakes as follows:
	\begin{align*}
		M_1 + &M_h + M_S \leq M_1 + M_h + 2(|E_1| - M_1 + |E_h| - M_h) \\
		&= 2 |E_1| + 2 |E_h| - |M_1| - |M_h| \leq 2 |E_1| + \frac{3}{2} |E_h| \\
		&= \sum_{(i,j) \in E_1} 2x_{ij} + \sum_{(i,j) \in E_h} 3x_{ij} \\
		&\leq 3 \sum_{(i,j) \in E} x_{ij} \leq 3 \text{OPT}_\mathit{CD}.
	\end{align*}
	Lemma~\ref{lem:piv} can similarly be used to show the same result in expectation for random pivot nodes.
\end{proof}
}

{\color{violet}
  The proof is quite informal (and there are several critical typos), so I rewrote it.
  The first paragraph can be moved to the end of section 1.
\begin{proof}
The key to our updated analysis is the following observation: for \emph{every} choice of pivot nodes, at most half of the edges in $E_W$ will end up inside the clusters formed by Algorithm~\ref{alg:mfp}. To see why, note that edges in $E_W$ come in pairs, since every open wedge $w \in W$ contains exactly two edges that end up in $E_W$. For an edge $e \in E_W$, let $p(e) \in E_W$ be the ``partner'' edge that came from the same open wedge in $W$ as $e$. Consider an edge $e = (i,j) \in E_W$ that ends up inside a cluster $C_k$ formed by pivoting on node $k$. The partner edge $p(e)$ must be incident to $i$ or $j$ but not both, since it forms an open wedge with $(i,j)$. Thus, $p(e)$ has one endpoint in $C_k$ but is not contained inside $C_k$ as this would imply $C_k$ is not a clique. Therefore, every edge $e \in E_W$ contained inside a cluster maps uniquely to an edge (its partner) that is between two clusters. This proves that at most half $|E_W|/2$ weak edges are inside clusters.

Let $M_W$ be the number of ``weak'' mistakes made by MFP, i.e., the number of weak edges between clusters. Let $M_S$ be the number of mistakes made at ``strong'' edges, i.e., edges in $E - E_W$ that are separated between clusters. By Lemma~\ref{lem:piv}, using Pivoting Strategy 1 or 2 on $\hat{G}$ guarantees that $M_S \leq 2(|E_W| - M_W)$. The total number of mistakes made by the algorithm is therefore bounded as follows:
\begin{align*}
	M_W + M_S &\leq M_W + 2(|E_W| - M_W) = 2|E_W| - M_W \\
 &\leq \frac{3}{2} |E_W| = 3 |W| \leq 3 \text{OPT}_{CD}.
\end{align*}
If we select pivot nodes uniformly at random, $M_W$ and $M_S$ become random variables, but coupling Lemma~\ref{lem:piv} with the observation that $M_W \leq |E_W|/2$ for every choice of pivot nodes provides the same guarantee in expectation.
\end{proof}
}
